ActionSwitch: Class-agnostic Detection of Simultaneous Actions in Streaming Videos

Online Temporal Action Localization (On-TAL) is a critical task that aims to instantaneously identify action instances in untrimmed streaming videos as soon as an action concludes -- a major leap from frame-based Online Action Detection (OAD). Yet, the challenge of detecting overlapping actions is often overlooked even though it is a common scenario in streaming videos. Current methods that can address concurrent actions depend heavily on class information, limiting their flexibility. This paper introduces ActionSwitch, the first class-agnostic On-TAL framework capable of detecting overlapping actions. By obviating the reliance on class information, ActionSwitch provides wider applicability to various situations, including overlapping actions of the same class or scenarios where class information is unavailable. This approach is complemented by the proposed "conservativeness loss", which directly embeds a conservative decision-making principle into the loss function for On-TAL. Our ActionSwitch achieves state-of-the-art performance in complex datasets, including Epic-Kitchens 100 targeting the challenging egocentric view and FineAction consisting of fine-grained actions.

==> fig/arch.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{pic/arch_v12.pdf}
\vspace{-5mm}
\caption{
\textbf{Architecture.}
Features $\fVideo$ and $\fClass$ are generated by VLM video and text encoders from video frames and action names, respectively
The action localizer detects class-agnostic action instances, and their features ($\fAction$) are extracted using RoI-Align. 
Cosine similarities between $\fAction$ and $\fClass$ are computed to assign the top-scoring category to each action instance.
The category score ($s_c$) is averaged with its actionness score ($s_a$) to obtain the final confidence score ($s$).
}
\vspace{-3mm}
\label{fig:arch}
\end{figure}


==> fig/motivation.tex <==

\begin{figure}[t!]
\centering
\includegraphics[width=0.6\linewidth]{pic/motivation_v11}
% \vspace{-5mm}
\caption{
% \textbf{Effectiveness of pseudo-labels.}
\textbf{Effectiveness of self-training for OV-TAL.}
% Localization accuracy comparison based on the use of pseudo-labels obtained from unlabeled videos.
When training a class-agnostic action localizer with human-labels of base categories (GT), a significant recall decrease is observed during training ($5 \rightarrow 15$). 
The utilization of pseudo-labels from unlabeled videos (GT+PL) prevents this problem and improves the localization of unseen actions.
The experiment is conducted within the 50-50\% ZS-TAL setting of THUMOS14~\cite{idrees2017thumos14}.
}
\vspace{-3mm}
\label{fig:motivation}
\end{figure}

==> fig/overview.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{pic/overview_v3}
\vspace{-5mm}
\caption{
\textbf{Our self-training pipeline.}
In \textbf{step (a)}, a class-agnostic action localizer is trained using human-annotated closed-vocabulary TAL datasets.
Then, it generates pseudo action instances on unlabeled, large-scale videos, where the semantics of actions are open.
In \textbf{step (b)}, the merged dataset is used to train the open-world action localizer, capable of localizing any action instance.
% Then, the trained localizer is used for OV-TAL with the open-vocabulary action classifier based on VLMs.
Then, the trained localizer is used for OV-TAL with the open-vocabulary action classifier based on VLMs.
}
\vspace{-3mm}
\label{fig:overview}
\end{figure}


==> fig/ovtal_setting.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{pic/ovtal_setting_v5.pdf}
\vspace{-5mm}
\caption{
\textbf{Comparison of ZS-TAL and OV-TAL settings.}
In ZS-TAL, a training dataset is confined to $\mathcal{C}_{train}$ which is strictly separated from $\mathcal{C}_{test}$, the test-time categories.
OV-TAL allows the use of \textit{unlabeled} videos which may contain a part of $\mathcal{C}_{test}$.
}
\vspace{-3mm}
\label{fig:ovtal_setting}
\end{figure}


==> fig/pl_quality.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{pic/pl_score-tiou_v2.pdf}
% \vspace{-5mm}
\caption{
% \textbf{Quality analysis of pseudo-labels on THUMOS14 and FineAction.}
\textbf{Quality analysis of pseudo-labels.}
Correlation between the actionness of pseudo-labels and their tIoU between GT instances is measured on THUMOS14 and FineAction.
The left graphs show the average of tIoU values in each interval of actionness (0.1).
The right graphs show the scatter plot.
}
\vspace{-3mm}
\label{fig:pl_quality}
\end{figure}

==> fig/pl_scalability.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{pic/pl_scalability_v5.pdf}
\vspace{-2mm}
\caption{
% \textbf{Quality analysis of pseudo-labels on THUMOS14 and FineAction.}
\textbf{Scalability analysis with random videos.}
The blue dotted lines show the self-training results using the FineAction training videos for novel categories ($\mathcal{D}_{N}$).
Even with random videos, the self-training can achieve $\text{mAP}_{N}$ of that based on $\mathcal{D}_{N}$.
Both $\text{mAP}_{A}$ and $\text{mAP}_{B}$ increase by scaling up the volume of videos.
}
\vspace{-3mm}
\label{fig:pl_scalability}
\end{figure}

==> fig/pl_sensitivity.tex <==
\begin{figure}[t!]
\centering
% \includegraphics[width=\linewidth]{pic/pl_sensitivity_v5.jpg}
\includegraphics[width=\linewidth]{pic/pl_sensitivity_v7.pdf}
% \vspace{-5mm}
\caption{
\textbf{Sensitivity analysis of pseudo-labels in self-training.}
Our self-training using pseudo-labels is robust against the threshold values after removing very low-confident noisy predictions (\eg, at 0.1).
% The experiment is conducted on FineAction~\cite{liu2022fineaction}.
The experiment is conducted on FineAction.
}
\vspace{-3mm}
\label{fig:pl_sensitivity}
\end{figure}

==> table/abl_module.tex <==

\begin{table}[b!]
\centering
\resizebox{0.6\linewidth}{!}{
    \begin{tabular}{@{}l|cc@{}}
    \toprule
    Method & F1 (\%) $\uparrow$ & Recall (\%) $\uparrow$ \\
    \midrule
    \multicolumn{3}{c}{Thumos14} \\
    \midrule
    base-2s & 42.03 & 53.63  \\
    conserv-2s & 49.62 & 52.53  \\
    base-4s & 44.05 & 58.84  \\
    conserv-4s & 52.36 & 58.04  \\
    \midrule
    \multicolumn{3}{c}{FineAction} \\
    \midrule
    base-2s & 16.04 & 20.09  \\
    conserv-2s & 17.23 & 17.98  \\
    base-4s & 16.54 & 22.07  \\
    conserv-4s & 18.70 & 20.09 \\
    \bottomrule
\end{tabular}
}
\vspace{1mm}
\caption{Ablation studies}
\label{tab:my_label}
\end{table}

==> table/fineaction_oad_full.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}l |ccccc ccccc | c c @{}}
\toprule[2pt]
\multirow{2}{*}{Method} & \multicolumn{10}{c|}{Offsets} & \multirow{2}{*}{\# proposal} & \multirow{2}{*}{\# GT}\\ \cline{2-11} 
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 &  \\
\toprule[1.5pt]
CAG-QIL~\cite{cagqil} & 6.33 & 8.86 & 10.41 & 11.49 & 12.63 & 13.44 & 14.13 & 14.66 & 25.34 & 15.77 & 15138 & 24236 \\
SimOn~\cite{simon} & 9.08 & 13.33 & 16.30 & 18.70 & 20.33 & 21.55 & 22.75 & 23.86 & 24.90 & 26.01 & 58956 & 24236 \\
\textbf{ActionSwitch (Ours)} & 9.35 & 13.26 & 15.38 & 17.01 & 18.22 & 19.11 & 19.92 & 20.63 & 21.24 & 21.92 & 29236 & 24236  \\
\bottomrule[2pt]
\end{tabular}%
}
\vspace{1mm}
\caption{Comparison of other state-of-the-art ODAS methods on FineAction dataset~\cite{fineaction}. 
% As Kinetics pretrained features are utilized in all three models, reported \textit{m}AP is much higher than those in the original papers~\cite{cagqil, simon}. 
For each metric, the best is bolded.
}
\label{tab:odas}
\end{table*}


==> table/fineaction_tiou_abl.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{@{} c|c | l | ccccc | ccccc | c @{}}
    \toprule[2pt]
    \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}{c} Setting \end{tabular}}} & \multirow{2}{*}{\begin{tabular}{@{}l@{}}Method\end{tabular}} & \multicolumn{5}{c|}{F1} & \multicolumn{5}{c|}{Recall} & \multirow{2}{*}{\begin{tabular}{c} \# proposal \end{tabular}} \\
    \multicolumn{2}{c|}{} & & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & \\
    \toprule[1.5pt]

    \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}{c} Offline\\TAL\end{tabular}}} & ActionFormer~\cite{actionformer} & 4.49 & 4.12 & 3.62 & 2.98 & 2.23 & \textbf{77.84} & \textbf{71.42} & \textbf{62.83} & \textbf{51.60} & \textbf{38.72} & 816100 \\ % TSN feature
    \multicolumn{2}{c|}{} & ActionFormer\textsuperscript{\textdagger}~\cite{actionformer} & \textbf{38.10} & \textbf{34.59} & \textbf{30.14} & \textbf{24.90} & \textbf{18.84} & 31.92 & 28.97 & 25.25 & 20.86 & 15.78 & 16369 \\
    
    \midrule[1pt]
    
    \multirow{5}{*}{\begin{tabular}{c} Online\\TAL\end{tabular}} & \multirow{2}{*}{TAL-Extension}  & OAT (\textit{downsampled by 4})~\cite{oat} & \textbf{25.54} & \textbf{22.86} & \textbf{18.64} & \textbf{13.17} & \textbf{7.98} & \textbf{52.20} & \textbf{46.72} & \textbf{38.10} & \textbf{26.92} & \textbf{16.30} & 74823 \\
    & & OAT~\cite{oat} & 11.38 & 9.38 & 7.21 & 5.23 & 3.26 & 12.85 & 10.60 & 8.14 & 5.90 & 3.69 & 30496 \\
    \cdashline{2-14}
    \noalign{\vskip 0.5ex}
    & \multirow{3}{*}{OAD-Extension} & CAG-QIL~\cite{cagqil} & 24.15 & 19.89 & 15.67 & 12.08 & 8.90 & 19.62 & 16.15 & 12.73 & 9.82 & 7.23 & 15138 \\
    & & SimOn~\cite{simon} & 17.29 & 13.93 & 10.53 & 7.69 & 5.24 & 29.68 & 23.90 & 18.06 & 13.20 & 9.00 & 58956 \\
    & & \textbf{ActionSwitch (Ours)} & \textbf{29.80} & \textbf{24.97} & \textbf{19.43} & \textbf{14.55} & \textbf{10.08} & \textbf{33.37} & \textbf{27.96} & \textbf{21.76} & \textbf{16.29} & \textbf{11.28} & 29972 \\
    \bottomrule[2pt]
\end{tabular}
}
\vspace{0.5mm}
\caption{
Comparison to other TAL methods on FineAction dataset~\cite{fineaction}. The number of ground truth proposals is 24236.
% All results are measured with the features extracted from the Kinetics~\cite{i3d} pre-trained TSN~\cite{tsn} model. We report \textit{m}AP at different tIoU thresholds and average \textit{m}AP in [0.3:0.1:0.7]. 
% In the offline TAL results, \textsuperscript{\textdagger} indicates the results with the optimal threshold that drops the low-confidence proposals and achieves the best F1 score.
% For each metric, the best is bolded.
}
\label{tab:fineaction_f1}
\end{table*}


==> table/human_perception_eval.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
    \begin{tabular}{@{} c|ccccc ccccc | c @{}}    
    \toprule[2pt]
    Video ID & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & Avg. \\
    \toprule[1.5pt]
    Preference (\%) & 98.33 & 93.33 & 93.33 & 91.67 & 95.00 & 98.33 & 96.67 & 98.33 & 95.00 & 96.67 & 95.67 \\
    \bottomrule[2pt]
    \end{tabular}
}
\vspace{2mm}
\caption{Human preference results. ``Preference'' here denotes preference of F1-best detection results over mAP counterpart.}
\label{tab:human_eval}
\end{table}

==> table/multithomus.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|c|c}
\toprule[2pt]
\# switch & F1@0.5 & precision@0.5 & recall@0.5 & \# proposal & \# gt                \\ \midrule[1pt]
1            & 16.51  & \textbf{42.85}         & 10.22      & 4816      & \multirow{4}{*}{20186} \\
2            & 30.82  & 34.37         & 27.94      & 16405     &                        \\ 
3            & \textbf{32.76} & 30.04         & 36.02      & 24211     &                        \\ 
4            & 29.25  & 22.67         & \textbf{41.21}      & 36682     &                        \\ \bottomrule[2pt]
\end{tabular}%
}
\caption{Multiple switch configurations tested in Multithumos \cite{multithumos} dataset. Conservativeness loss ($\alpha=0.025$) is also posed to regularize excessive proposals. A good F1 score is observed when the number of generated predictions (\# proposal) is close to the number of ground truth instances (\# gt).}
\vspace{-3mm}
\label{tab:multithumos}
\end{table}

==> table/muses_tal.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.9\linewidth}{!}{
    \begin{tabular}{@{} c|c | l| ccc |cccccc@{}}
    \toprule[2pt]
    \multicolumn{2}{c|}{Setting} & Method & F1 & Recall & Precision & mAP@0.3 & 0.4 & 0.5 & 0.6 & 0.7 & Avg. \\
    \toprule[1.5pt]
    \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}{c} Offline\\TAL \end{tabular}}} & ActionFormer~\cite{actionformer} & 7.27 & \textbf{90.65} & 3.79 & \textbf{27.57} & \textbf{24.07} & \textbf{19.74} & \textbf{15.63} & \textbf{11.32} & \textbf{19.67} \\
    \multicolumn{2}{c|}{} & ActionFormer\textsuperscript{\textdagger}~\cite{actionformer} & \textbf{54.00} & 49.05 & \textbf{60.05} & 18.86 & 16.47 & 13.74 & 11.27 & 8.45 & 13.76 \\
    \midrule[1pt]
    \multirow{5}{*}{\begin{tabular}{c} Online\\TAL\end{tabular}} & \multirow{1}{*}{N/A} & OAT~\cite{oat} & \textbf{37.47} & \textbf{66.76} & \textbf{26.04} & \textbf{22.09} & \textbf{18.54} & \textbf{14.20} & \textbf{8.89} & \textbf{4.70} & \textbf{13.68} \\
    \cdashline{2-12}
    \noalign{\vskip 0.5ex}
    & \multirow{4}{*}{State-Aware} & CAG-QIL~\cite{cagqil} & 32.48 & 24.68 & \textbf{47.47} & 5.01 & 3.42 & 2.83 & 2.13 & 1.34 & 2.94 \\
    & & SimOn~\cite{simon} & 25.59 & 38.54 & 19.15 & 11.09 & 8.17 & 5.92 & 3.89 & 2.37 & 6.29 \\
    & & \textbf{ActionSwitch -- 4S (Ours)} & 33.87 & 30.93 & 37.42 & 11.68 & 9.11 & 6.51 & 4.60 & 2.96 & 6.97 \\
    & & \textbf{ActionSwitch -- 5S (Ours)} & \textbf{37.79} & \textbf{42.02} & 34.32 & \textbf{14.35} & \textbf{11.19} & \textbf{7.70} & \textbf{5.22} & \textbf{3.01} & \textbf{8.29} \\
    \bottomrule[2pt]
\end{tabular}
}
\vspace{1mm}
\caption{Comparison to other TAL methods on MUSES dataset~\cite{muses}. We report \textit{m}AP at different tIoU thresholds and average \textit{m}AP in [0.3:0.1:0.7]. 
\textsuperscript{\textdagger} indicates the results with the optimal threshold that drops the low-confidence proposals and achieves the best F1 score.
For each metric, the best is bolded.
}
\label{tab:fineaction_main}
\end{table*}


% \begin{table*}[t!]
% \centering
% \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{@{} c|c | l| cc|cccccc@{}}
%     \toprule[2pt]
%     \multicolumn{2}{c|}{Setting} & Method & F1 & Recall & mAP@0.3 & 0.4 & 0.5 & 0.6 & 0.7 & Avg. \\
%     \toprule[1.5pt]
%     \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}{c} Offline\\TAL \end{tabular}}} & ActionFormer~\cite{actionformer} & 7.27 & \textbf{90.65} & \textbf{27.57} & \textbf{24.07} & \textbf{19.74} & \textbf{15.63} & \textbf{11.32} & \textbf{19.67} \\
%     \multicolumn{2}{c|}{} & ActionFormer\textsuperscript{\textdagger}~\cite{actionformer} & \textbf{54.00} & 49.05 & 18.86 & 16.47 & 13.74 & 11.27 & 8.45 & 13.76 \\
%     \midrule[1pt]
%     \multirow{4}{*}{\begin{tabular}{c} Online\\TAL\end{tabular}} & \multirow{1}{*}{N/A} & OAT~\cite{oat} & \textbf{37.47} & \textbf{66.76} & \textbf{22.09} & \textbf{18.54} & \textbf{14.20} & \textbf{8.89} & \textbf{4.70} & \textbf{13.68} \\
%     \cdashline{2-11}
%     \noalign{\vskip 0.5ex}
%     & \multirow{3}{*}{State-Aware} & CAG-QIL~\cite{cagqil} & 32.48 & 24.68 & 5.01 & 3.42 & 2.83 & 2.13 & 1.34 & 2.94 \\
%     & & SimOn~\cite{simon} & 25.59 & 38.54 & 11.09 & 8.17 & 5.92 & 3.89 & 2.37 & 6.29 \\
%     & & \textbf{ActionSwitch -- 4S (Ours)} & 33.87 & 30.93 & 11.68 & 9.11 & 6.51 & 4.60 & 2.96 & 6.97 \\
%     & & \textbf{ActionSwitch -- 5S (Ours)} & \textbf{37.79} & \textbf{42.02} & \textbf{14.35} & \textbf{11.19} & \textbf{7.70} & \textbf{5.22} & \textbf{3.01} & \textbf{8.29} \\
%     \bottomrule[2pt]
% \end{tabular}
% }
% \vspace{1mm}
% \caption{Comparison to other TAL methods on MUSES dataset~\cite{muses}. We report \textit{m}AP at different tIoU thresholds and average \textit{m}AP in [0.3:0.1:0.7]. 
% \textsuperscript{\textdagger} indicates the results with the optimal threshold that drops the low-confidence proposals and achieves the best F1 score.
% For each metric, the best is bolded.
% }
% \label{tab:fineaction_main}
% \end{table*}



==> table/muses_tiou_abl.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{@{} c|c | l | ccccc | ccccc | c @{}}
    \toprule[2pt]
    \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}{c} Setting \end{tabular}}} & \multirow{2}{*}{\begin{tabular}{@{}l@{}}Method\end{tabular}} & \multicolumn{5}{c|}{F1} & \multicolumn{5}{c|}{Recall} & \multirow{2}{*}{\begin{tabular}{c} \# proposal \end{tabular}} \\
    \multicolumn{2}{c|}{} & & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & \\
    \toprule[1.5pt]

    \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}{c} Offline\\TAL\end{tabular}}} & ActionFormer~\cite{actionformer} & 7.80 & 7.62 & 7.27 & 6.67 & 5.76 & 97.24 & 94.99 & 90.65 & 83.15 & 71.85 & 222000\\ % TSN feature
    \multicolumn{2}{c|}{} & ActionFormer\textsuperscript{\textdagger}~\cite{actionformer} & \textbf{62.81} & \textbf{59.12} & \textbf{54.00} & \textbf{47.90} & \textbf{40.97} & \textbf{57.06} & \textbf{53.71} & \textbf{49.05} & \textbf{43.51} & \textbf{37.22} & 7579 \\
    
    \midrule[1pt]
    
    \multirow{5}{*}{\begin{tabular}{c} Online\\TAL\end{tabular}} & \multirow{1}{*}{TAL-Extension} & OAT~\cite{oat} & \textbf{45.65} & \textbf{42.04} & \textbf{37.47} & \textbf{31.17} & \textbf{23.68} & \textbf{81.39} & \textbf{74.91} & \textbf{66.76} & \textbf{55.54} & \textbf{42.19} & 23786 \\
    \cdashline{2-14}
    \noalign{\vskip 0.5ex}
    & \multirow{4}{*}{OAD-Extension} & CAG-QIL~\cite{cagqil} & 45.77 & 39.24 & 32.48 & 25.51 & 19.98 & 34.78 & 29.82 & 24.68 & 19.39 & 15.19 & 4824 \\
    & & SimOn~\cite{simon} & 35.93 & 30.89 & 25.59 & 20.26 & 15.61 & 54.12 & 46.53 & 38.54 & 30.51 & 23.52 & 18674 \\
    & & \textbf{ActionSwitch -- 4S (Ours)} & 46.52 & 40.83 & 33.87 & 26.88 & 20.39 & 42.49 & 37.29 & 30.93 & 24.55 & 18.62 & 7670 \\
    & & \textbf{ActionSwitch -- 5S (Ours)} & \textbf{51.84} & \textbf{45.68} & \textbf{37.79} & \textbf{30.22} & \textbf{22.47} & \textbf{57.65} & \textbf{50.81} & \textbf{42.02} & \textbf{33.61} & \textbf{25.00} & 11359 \\
    \bottomrule[2pt]
\end{tabular}
}
\vspace{0.5mm}
\caption{
Comparison to other TAL methods on MUSES dataset \cite{muses}. \textbf{4S} and \textbf{5S} denote 4-state and 5-state settings respectively. The number of ground truth proposals is 9278.
% All results are measured with the features extracted from the Kinetics~\cite{i3d} pre-trained TSN~\cite{tsn} model. We report \textit{m}AP at different tIoU thresholds and average \textit{m}AP in [0.3:0.1:0.7]. 
% In the offline TAL results, \textsuperscript{\textdagger} indicates the results with the optimal threshold that drops the low-confidence proposals and achieves the best F1 score.
% For each metric, the best is bolded.
}
\label{tab:muses_f1}
\end{table*}


==> table/tal_same_classifier.tex <==
\begin{table}[t!]
\centering
\resizebox{0.9\linewidth}{!}{
    \begin{tabular}{ll|c|c|ccc}
    \toprule[2pt]
    % Dataset & \multicolumn{2}{c|}{Method} &  Avg. mAP \\
    
    % Method & Classifier &  Avg. mAP (THUMOS14) & Avg. mAP (FineAction)\\

    \multirow{2}{*}{Method} & \multirow{2}{*}{Classifier} & \multicolumn{2}{c}{Avg. mAP} & \multicolumn{2}{c}{SA} & \multicolumn{2}{c}{O} & \multicolumn{2}{c}{V}
    % \cline{3-4}
    % \noalign{\vskip 0.5ex}
     & & THUMOS14 & FineAction & & \\
    
    \toprule[1.5pt]
    
    \multicolumn{2}{l|}{\textbf{ActionSwitch (Ours)}} & 39.7 & 5.36 \\ 
    \cline{1-4}
    \noalign{\vskip 0.5ex}
    
    CAG-QIL & Ours & 33.1 & 4.45 \\
    \cline{1-4}
    \noalign{\vskip 0.5ex}
    
    \multirow{2}{*}{SimOn} & Ours & 34.4 & 3.51 \\
     & Official & 33.0 & 4.12 \\
    \cline{1-4}
    \noalign{\vskip 0.5ex}
    
    \multirow{2}{*}{OAT} & Ours & 45.5 & 0.97 \\
     & Official & 45.3 & 0.34 \\

    \bottomrule[2.0pt]
    \end{tabular}
}
\caption{Average mAP results using the same classifier. 
Since CAG-QIL doesn't provide the official code, we report the reproduced results which are higher than the values from the paper.
% For CAG-QIL, we only have reproduced results. (higher than the reported mAP in the original CAG-QIL paper)
}
\vspace{1mm}
\label{tab:tal_same_classifier}
\vspace{-8mm}
\end{table}

% \begin{table}[t!]
% \centering
% \resizebox{0.68\linewidth}{!}{
%     \begin{tabular}{c|ll|c}
%     \toprule[2pt]
%     % Dataset & \multicolumn{2}{c|}{Method} &  Avg. mAP \\
%     Dataset & Method & Classifier &  Avg. mAP \\
%     \toprule[1.5pt]
    
%     \multirow{6}{*}{\begin{tabular}{c} THUMOS14 \end{tabular}} 
%     & \multicolumn{2}{l|}{\textbf{ActionSwitch (Ours)}} & 39.7 \\ 
%     \cline{2-4}
%     \noalign{\vskip 0.5ex}

%     & CAG-QIL & Ours & 33.1 \\
%     \cline{2-4}
%     \noalign{\vskip 0.5ex}
    
%     & \multirow{2}{*}{SimOn} & Ours & 34.4 \\
%     &  & Official & 33.0 \\
%     \cline{2-4}
%     \noalign{\vskip 0.5ex}
    
%     & \multirow{2}{*}{OAT} & Ours & 45.5 \\
%     &  & Official & 45.3 \\
    
%     \midrule[1pt]

%     \multirow{6}{*}{\begin{tabular}{c} FineAction \end{tabular}} 
%     & \multicolumn{2}{l|}{\textbf{ActionSwitch (Ours)}} & 5.36 \\ 
%     \cline{2-4}
%     \noalign{\vskip 0.5ex}

%     & CAG-QIL & Ours & 4.45 \\
%     \cline{2-4}
%     \noalign{\vskip 0.5ex}
    
%     & \multirow{2}{*}{SimOn} & Ours & 3.51 \\
%     &  & Official & 4.12 \\
%     \cline{2-4}
%     \noalign{\vskip 0.5ex}
    
%     & \multirow{2}{*}{OAT} & Ours & 0.97 \\
%     &  & Official & 0.34 \\

%     \bottomrule[2.0pt]
%     \end{tabular}
% }
% \caption{Average mAP results using the same classifier. 
% Since CAG-QIL doesn't provide the official code, we report the reproduced results which are higher than the values from the paper.
% % For CAG-QIL, we only have reproduced results. (higher than the reported mAP in the original CAG-QIL paper)
% }
% \vspace{1mm}
% \label{tab:tal_same_classifier}
% \vspace{-8mm}
% \end{table}

==> table/tal_same_classifier2.tex <==
\newcommand{\cx}{\ding{55}}
\newcommand{\cy}{\ding{51}}
\newcommand{\cc}{\ding{61}}

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc|cc|c|c|c}
\toprule[2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} &
  \multirow{2}{*}{Classifier} &
  \multicolumn{2}{c|}{Avg. mAP} &
  \multirow{2}{*}{SA} &
  \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}Class \\ Agnostic\end{tabular}}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Detect Overlapping \\ Instances\end{tabular}} \\ \cline{3-4}
\multicolumn{1}{c|}{}      &             & \multicolumn{1}{c|}{THUMOS14} & FineAction &                    &                    &                    \\ \hline
\multicolumn{2}{c|}{\textbf{ActionSwitch (Ours)}} & \multicolumn{1}{c|}{39.7}     & 5.36       & \cy                  & \cy                  & \cy                  \\ \hline
CAG-QIL~[\textcolor{green}{15}]                    & Ours        & \multicolumn{1}{c|}{33.1}     & 4.45       & \cy                 & \cy                  &                   \\ \hline
\multirow{2}{*}{SimOn~[\textcolor{green}{35}]}     & Ours        & \multicolumn{1}{c|}{34.4}     & 3.51       & \multirow{2}{*}{\cy} & \multirow{2}{*}{} & \multirow{2}{*}{\bigtriangleup} \\
                           & Official    & \multicolumn{1}{c|}{33.0}     & 4.12       &                    &                    &                    \\ \hline
\multirow{2}{*}{OAT~[\textcolor{green}{18}]}       & Ours        & \multicolumn{1}{c|}{45.5}     & 0.97       & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{\cy} \\
                           & Official    & \multicolumn{1}{c|}{45.3}     & 0.34       &                    &                    &                    \\ \bottomrule[2.0pt]
\end{tabular}%

}
\caption{Average mAP results using the same classifier. 
%Since CAG-QIL doesn't provide the official code, we report the reproduced results which are higher than the values from the paper.
For CAG-QIL, we only have reproduced results as there is no official code. (higher than the reported mAP in the original CAG-QIL paper)
}
\label{tab:tal_same_classifier2}
% \vspace{-8mm}
\vspace{-5mm}
\end{table}

==> table/thumos14_oad_full.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}l |ccccc ccccc | c c @{}}
\toprule[2pt]
\multirow{2}{*}{Method} & \multicolumn{10}{c|}{Offsets} & \multirow{2}{*}{\# detection} & \multirow{2}{*}{\# GT}\\ \cline{2-11} 
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 &  \\
\toprule[1.5pt]
CAG-QIL~\cite{cagqil} & 28.30 & 42.86 & 50.12 & 54.27 & 57.00 & 58.22 & 59.77 & 60.33 & 61.03 & 61.50 & 4026 & 3358 \\
SimOn~\cite{simon} & 31.45 & 46.22 & 54.11 & \textbf{59.68} & \textbf{62.69} & \textbf{65.07} & \textbf{66.73} & \textbf{67.71} & \textbf{69.25} & \textbf{69.93} & 10086 & 3358 \\
\textbf{ActionSwitch (Ours)} & \textbf{33.06} & \textbf{47.06} & \textbf{54.44} & 58.74 & 61.13 & 62.82 & 63.74 & 64.71 & 65.34 & 66.02 & 4091 & 3358 \\
\bottomrule[2pt]
\end{tabular}%
}
\vspace{1mm}
\caption{Comparison of other state-of-the-art ODAS methods on THUMOS14 dataset~\cite{THUMOS14}. 
As Kinetics pretrained features are utilized in all three models, reported \textit{m}AP is much higher than those in the original papers~\cite{cagqil, simon}. 
For each metric, the best is bolded.
}
\label{tab:odas}
\end{table*}


% \begin{table*}[t!]
% \centering
% \resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{@{}l |ccccc ccccc | c c @{}}
% \toprule[2pt]
% \multirow{2}{*}{Method} & \multicolumn{10}{c|}{Offsets} & \multirow{2}{*}{\# proposal} & \multirow{2}{*}{\# GT}\\ \cline{2-11} 
%  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 &  \\
% \toprule[1.5pt]
% CAG-QIL~\cite{cagqil} & 28.30 & 42.86 & 50.12 & 54.27 & 57.00 & 58.22 & 59.77 & 60.33 & 61.03 & 61.50 & 4026 & 3358 \\
% SimOn~\cite{simon} & 31.45 & 46.22 & 54.11 & 59.68 & 62.69 & 65.07 & 66.73 & 67.71 & 69.25 & 69.93 & 10086 & 3358 \\
% \textbf{ActionSwitch (Ours)} & 33.06 & 47.06 & 54.44 & 58.74 & 61.13 & 62.82 & 63.74 & 64.71 & 65.34 & 66.02 & 4091 & 3358 \\
% \bottomrule[2pt]
% \end{tabular}%
% }
% \vspace{1mm}
% \caption{Comparison of other state-of-the-art ODAS methods on THUMOS14 dataset~\cite{thumos14}. 
% As Kinetics pretrained features are utilized in all three models, reported \textit{m}AP is much higher than those in the original papers~\cite{cagqil, simon}. 
% For each metric, the best is bolded.
% }
% \label{tab:odas}
% \end{table*}


==> table/thumos14_tiou_abl.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{@{} c|c | l | ccccc | ccccc | c @{}}
    \toprule[2pt]
    \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}{c} Setting \end{tabular}}} & \multirow{2}{*}{\begin{tabular}{@{}l@{}}Method\end{tabular}} & \multicolumn{5}{c|}{F1} & \multicolumn{5}{c|}{Recall} & \multirow{2}{*}{\begin{tabular}{c} \# proposal \end{tabular}} \\
    \multicolumn{2}{c|}{} & & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & \\
    \toprule[1.5pt]

    \multicolumn{2}{c|}{\multirow{6}{*}{\begin{tabular}{c} Offline\\TAL\end{tabular}}} & G-TAD~\cite{gtad} & 7.11 & 6.88 & 6.36 & 5.60 & 4.52 & 93.21 & 90.29 & 83.38 & 73.50 & 59.29 & 84752 \\ 
    \multicolumn{2}{c|}{} & TadTR~\cite{tadtr} & 3.91 & 3.77 & 3.54 & 3.21 & 2.70 & 97.28 & 93.78 & 88.07 & 79.73 & 67.23 & 161341\\  
    \multicolumn{2}{c|}{} & ActionFormer~\cite{actionformer} & 14.30 & 14.17 & 13.80 & 12.94 & 11.31 & \textbf{97.41} & \textbf{96.55} & \textbf{94.01} & \textbf{88.18} & \textbf{77.04} & 42400 \\ % TSN feature
    \multicolumn{2}{c|}{} & G-TAD\textsuperscript{\textdagger}~\cite{gtad} & 61.34 & 57.26 & 51.07 & 44.10 & 35.41 & 59.95 & 55.96 & 49.91 & 43.09 & 34.60 & 3205\\ 
    \multicolumn{2}{c|}{} & TadTR\textsuperscript{\textdagger}~\cite{tadtr} & 75.67 & 72.81 & 68.42 & 60.64 & 50.04 & 69.65 & 67.02 & 62.97 & 55.81 & 46.06 & 2784\\ 
    \multicolumn{2}{c|}{} & ActionFormer\textsuperscript{\textdagger}~\cite{actionformer} & \textbf{82.91} & \textbf{80.71} & \textbf{75.47} & \textbf{68.26} & ]\textbf{57.00} & 80.91 & 78.77 & 73.65 & 66.62 & 55.63 & 3196 \\
    \midrule[1pt]
    
    \multirow{4}{*}{\begin{tabular}{c} Online\\TAL\end{tabular}} & TAL-Extension & OAT~\cite{oat} & \textbf{73.84} & \textbf{69.90} & \textbf{62.87} & \textbf{53.07} & \textbf{38.10} & \textbf{82.58} & \textbf{78.17} & \textbf{70.31} & \textbf{59.35} & \textbf{42.62} & 4153\\
    \cdashline{2-14}
    \noalign{\vskip 0.5ex}
    & \multirow{3}{*}{OAD-Extension} & CAG-QIL~\cite{cagqil} & 60.94 & 53.90 & 45.80 & 36.95 & 28.79 & 67.00 & 59.26 & 50.36 & 40.62 & 31.66 & 4026 \\
    & & SimOn~\cite{simon} & 39.32 & 34.82 & 28.73 & 22.85 & 16.52 & 71.28 & 63.11 & 52.09 & 41.42 & 29.95 & 8811 \\ % simon feature
    & & \textbf{ActionSwitch (Ours)} & \textbf{67.20} & \textbf{61.11} & \textbf{53.20} & \textbf{43.58} & \textbf{34.01} & \textbf{75.90} & \textbf{69.03} & \textbf{60.10} & \textbf{49.23} & \textbf{38.42} & 4228 \\
    \bottomrule[2pt]
\end{tabular}
}
\vspace{0.5mm}
\caption{
Comparison to other TAL methods on THUMOS14 dataset \cite{THUMOS14}. The number of ground truth proposals is 3358.
% All results are measured with the features extracted from the Kinetics~\cite{i3d} pre-trained TSN~\cite{tsn} model. We report \textit{m}AP at different tIoU thresholds and average \textit{m}AP in [0.3:0.1:0.7]. 
% In the offline TAL results, \textsuperscript{\textdagger} indicates the results with the optimal threshold that drops the low-confidence proposals and achieves the best F1 score.
% For each metric, the best is bolded.
}
\label{tab:thumos_f1}
\end{table*}

